Optimizer Benchmarking Needs to Account for Hyperparameter Tuning

The performance of optimizers, particularly in deep learning, depends considerably on their chosen hyperparameter configuration. The efficacy of optimizers is often studied under near-optimal problem-specific hyperparameters, and finding these settings may be prohibitively costly for practitioners. In this work, we argue that a fair assessment of optimizers' performance must take the computational cost of hyperparameter tuning into account, i.e., how easy it is to find good hyperparameter configurations using an automatic hyperparameter search. Evaluating a variety of optimizers on an extensive set of standard datasets and architectures, our results indicate that Adam is the most practical solution, particularly in low-budget scenarios.

==> alpha.tex <==

\section{\texorpdfstring{$\alpha$} -- tunability}
We provide additional methods to analyze tunability here. Let $p(t)$ denote the best performance observed after using budget $t$ of hyperparameter optimization algorithm. We call an optimizer $\alpha$-tunable ($\alpha \in [0,1]$) at $t$ if $p(t) \geq \alpha \cdot p(T)$. Thus $\alpha-$tunability is the ratio of number of times the neural network needs to be retrained with optimizer's hyperparameters being provided by an automatic method, to the total budget $T$ (maximum number of configurations tested).

For each optimizer, we define its \emph{$\alpha$-tunability} $\zeta(\alpha) = \frac{t}{T}$ for $\alpha \in \{0.9, 0.95, 0.99\}$.  This metric provides an intuitive and simple quantification of how easy it is to tune an optimizer to reach requisite performance. We extend $\alpha$--tunability to indicate the sharpness of the minima by computing the difference $\Delta = \zeta(\alpha_1) - \zeta(\alpha_2)$ where $\alpha_1 > \alpha_2$ and term it \emph{Sharpness}. In our experiments, we choose $\alpha_1 = 0.99$ and $\alpha_2 = 0.9$. Sharpness($\Delta$) is the relative time taken by the HPO to improve from $\alpha_2$ to $\alpha_1$ and thus quantifies the flatness of the minima in the space of hyperparameters. If the minima is sharper, then we expect random-search also takes a longer time to find it, thus the time required to go from $\alpha_1$ and $\alpha_2$ is higher. We provide Sharpness for our optimizers in table:\ref{tab:sharpness}.

\begin{table*}[ht]
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}lrrrrrrrrr@{}}
            \toprule
                             & \textbf{MNIST VAE} & \textbf{FMNIST 2C2D} & \textbf{CIFAR 100} & \textbf{CIFAR 10} & \textbf{SVHN WRN} & \textbf{IMDB LSTM} & \textbf{FMNIST VAE} & \textbf{Quadratic Deep} & \textbf{Char RNN} \\ \midrule
            \textbf{\Adagrad} & 92.0               & 99.0                 & 63.0               & 95.0              & \tb{10.0}         & 97.0               & 91.0                & 66.0                    & 95.0              \\
            \textbf{\Adam}    & 80.0               & 98.0                 & 40.0               & \tb{91.0}         & 71.0              & 93.0               & 90.0                & 75.0                    & 87.0              \\
            \textbf{\AdamLR} & 83.0               & 96.0                 & 71.0               & 94.0              & 98.0              & 70.0               & 95.0                & 93.0                    & 97.0              \\
            \textbf{\SGD}     & 98.0               & 95.0                 & 35.0               & 93.0              & 98.0              & 81.0               & 94.0                & \tb{6.0}                & 47.0              \\
            \textbf{\SGDM}    & \tb{58.0}          & 97.0                 & 50.0               & \tb{91.0}         & 59.0              & 72.0               & 90.0                & 30.0                    & 59.0              \\
            \textbf{\SGDMC}   & 95.0               & 83.0                 & 82.0               & 94.0              & 52.0              & 88.0               & \tb{75.0}           & 95.0                    & 87.0              \\
            \textbf{\SGDMCWC} & 94.0               & \tb{45.0}            & 78.0               & 95.0              & 98.0              & \tb{68.0}          & 88.0                & 16.0                    & 85.0              \\
            \textbf{\SGDMW}   & 65.0               & 97.0                 & \tb{23.0}          & 94.0              & 36.0              & 86.0               & 91.0                & 14.0                    & \tb{32.0} \\
            \bottomrule
        \end{tabular}
    }
    \caption{Sharpness for various optimizers examined.}
    \label{tab:sharpness}
\end{table*}


The above definition is not without faults. An optimizer's $\alpha$-tunability depends only on how fast it can get close to its \emph{own best performance}, a pitfall it shares with~\citet{probstTunabilityImportanceHyperparameters}. That is, an optimizer that peaks at the performance of a random classifier may be considered well-tunable because it reaches its peak performance in the first iteration. It is apparent from tables~\ref{tab:sharpness} and \ref{fig:perf_plots_app_full} that the top performance does not imply lower sharpness. Take the case of IMDB Bi-LSTM, the lowest sharpness is for \SGDMCWC, while the best performance is attained by \AdamLR, implying that \SGDMCWC settled to a minima faster which isn't necessarily better than the one \AdamLR found. In other terms, the flatness of the minima does not indicate how deep it is.


==> measuring_tunab.tex <==
Given the dichotomy of the problem of tunability, we argue that it needs to take into account
\begin{enumerate}
  \item how difficult it is to find a good hyperparameter configuration for the optimizer,
  \item the absolute performance of the optimizer.
\end{enumerate}
To see why both are needed, consider Figure~\ref{fig:probstillus}, which shows the performance in terms of loss of four different optimizers as a function of its only hyperparameter $\theta$ (by assumption). If we only consider requirement \#1, optimizer C would be considered the best, since every hyperparameter value is the optimum. However, its absolute performance is poor, making it of low practical value. Moreover, due to the same shape, optimizers A and B would be considered equally good, although optimizer A clearly outperforms B. On the other hand, if we only consider requirement \#2, optimizers B and D would be considered equally good, although optimizer D's optimum is harder to find.

As we show in Section~\ref{sec:related-work}, no existing definition of tunability takes both requirements into account. In the following, we present a formulation that does so.

\subsection{Preliminaries: hyperparameter optimization}
We define hyperparameter optimization (HPO) \citep{Feurer2019} as follows:
\begin{definition}
  Let $\mathcal{M}$ be an optimization algorithm with N hyperparameters $(\theta_1,\dots,\theta_N)\in\Theta$. Let a specific instantiation of $\mathcal{M}$ with $\boldsymbol{\theta}\in\Theta$ be denoted by $\mathcal{M}_{\boldsymbol{\theta}}$. Thus, given a dataset $D=D_{train}\bigcup D_{val}$, the following objective is minimized
  \begin{equation*}
    {\boldsymbol{\theta}}^\star = \arg\min_{\boldsymbol{\theta}\in\Theta} \mathcal{L}(\mathcal{M}_{\boldsymbol{\theta}}, D_{val})
  \end{equation*}
  where $\mathcal{M}_{\boldsymbol{\theta}}$ is trained on $D_{train}$. In our work, we use $\mathcal{L}$ to be validation loss.
\end{definition}
We use $\mathcal{L}(\boldsymbol{\theta})$ to refer to $\mathcal{L}(\mathcal{M}_{\boldsymbol{\theta}}, D_{val})$ for brevity. In our experiments, we use the time-tested Random Search~\citep{bergstra2012random} algorithm for HPO for simplicity.

\subsection{Defining tunability}
The ability to easily find good minima depends on the loss surface $\mathcal{L}$ itself. Thus, tunability is a characterization of the HPO's loss function $\mathcal{L}$. Here we present a quantification of this idea, which we illustrate with Figure~\ref{fig:optimillus}.

Let us assume that there are two optimizers E \& F, both with hyperparameter $\theta$, both of them used to minimize a function (e.g.\ train a neural network). Let the loss functions of HPO be $\mathcal{L}_E$ and $\mathcal{L}_F$ respectively. As the figure shows, the minimum of $\mathcal{L}_E$ is lower than that of $\mathcal{L}_F$ (denoted by $\theta_E^\star$ and $\theta_F^\star$) i.e. $\mathcal{L}_E(\theta_E^\star)< \mathcal{L}_F(\theta_F^\star)$.
\begin{figure}[htbp]
  \begin{subfigure}[t]{0.47\linewidth}
    \resizebox{\linewidth}{!}{
      \def\offset{-4}
      \begin{tikzpicture}[scale=0.5]
        \draw[thick,->] (0,0) -- (9.5,0);
        \node at (4.75, -.75) {Hyperparameter $\theta$};
        \draw[thick,->] (0,0) -- (0,13 + \offset);
        \node[rotate=90] at (-0.5, 4.5){Expected loss};
        \draw[myblue, very thick] (1,10 + \offset) to[out=0, in=105] (2, 8.5 + \offset);
        \draw[myblue, very thick] plot[smooth, domain=2:6] (\x, \x*\x - 8*\x + 20.5 + \offset);
        \draw[myblue, very thick] (6, 8.5 + \offset) to[out=75, in=180] (7, 10 + \offset)
        node[right] {\footnotesize Optimizer A};
        \draw[myviolet, very thick] (1,12 + \offset) to[out=0, in=100] (3, 10.5 + \offset);
        \draw[myviolet, very thick] plot[smooth, domain=3:5] (\x, 4*\x*\x - 32*\x + 70.5 + \offset);
        \draw[myviolet, very thick] (5, 10.5 + \offset) to[out=90, in=180] (7, 12 + \offset)
        node[right]{\footnotesize Optimizer D};
        \draw[myred, very thick] (1,12 + \offset) to[out=0, in=105] (2, 10.5 + \offset);
        \draw[myred, very thick] plot[smooth, domain=2:6] (\x, \x*\x - 8*\x + 22.5 + \offset);
        \draw[myred, very thick] (6, 10.5 + \offset) to[out=75, in=180] (7, 12 + \offset)
        node[above right] {\footnotesize Optimizer  B};
        \draw[mygreen, very thick] plot[domain=1:7](\x, 12.5 + \offset)%
        node[above right]{\footnotesize Optimizer C};
      \end{tikzpicture}}
    \caption{Illustration. It is important to consider both the absolute performance of optimizers as well as the tuning effort to get to good performances.}
    \label{fig:probstillus}
  \end{subfigure}
  \hspace{0.3cm}
  \begin{subfigure}[t]{0.47\linewidth}
    \resizebox{\textwidth}{!}{
      \begin{tikzpicture}[scale=0.5]
        \draw[thick,->] (0,0) -- (9.5,0);
        \node at (4.75, -.75) {Hyperparameter $\theta$};
        \draw[thick,->] (0,0) -- (0,9);
        \node[rotate=90] at (-0.5, 4.5){Expected loss $\mathcal{L}(\theta)$};
        \begin{scope}[yshift=1cm]
          \draw[RoyalPurple, very thick] (1,5) ..controls (3, 2) .. (7, 4) node[right] {\footnotesize Optimizer F};
          \draw[magenta, very thick] (1, 5.5) .. controls (4, 5) and (4, -1) .. (4.5, 3) to[out=85, in=190] (7, 4.5) node[right]{\footnotesize Optimizer E};
          \node[RoyalPurple,label={270:\color{RoyalPurple}{$\theta_F^\star$}},circle,fill,inner sep=2pt] at (3.25, 2.65) {};
          \node[magenta, label={270:\color{magenta}{$\theta_E^\star$}},circle,fill,inner sep=2pt] at (4.15, 1.65) {};
        \end{scope}
      \end{tikzpicture}}
    \caption{Illustration. While optimizer E can achieve the best performance after careful tuning, optimizer F is likely to provide better performance under a constrained HPO budget.}
    \label{fig:optimillus}
  \end{subfigure}
\end{figure}
However, the minimum of $\mathcal{L}_E$ is much sharper than that of $\mathcal{L}_F$, and in most regions of the parameter space F performs much better than E. This makes it easier to find configurations that already perform well. This makes optimizer F an attractive option when we have no prior knowledge of the good parameter settings.

The key-difference between the two interpretations is whether one prefers a `good enough' performance through fewer hyperparameter configuration searches (in the case of optimizer~F), or whether one is willing to spend computational time to get the best possible performance ($\theta^\star_E$ in the case of optimizer~E). In this work, we search for the hyperparameter through an HPO like Random Search. Thus, the difference of the two interpretations of tunability lies whether one values results from late stages of the HPO process (i.e. optimizer E is preferable due to better optimum) more than results from early stages of the HPO process (i.e. optimizer F is preferable).

Motivated by these observations, we propose the following metric for tunability.
\begin{definition}[$\omega$-tunability]
  Let $(\boldsymbol{\theta}_t, \mathcal{L}(\boldsymbol{\theta}_t))$ be the incumbents (best performance attained till $t$) of the HPO algorithm at iteration $t$ and $T$ be the hyperparameter tuning budget. For $w_t >0$ $\forall$ t and $\sum_t w_t < \infty$, we define $\omega$-tunability as  \[\omega\text{-tunability} = \sum_{t=1}^T \omega_t \mathcal{L}_t\]
\end{definition}
i.e, $\omega$-tunability is a weighted sum of the incumbents $\mathcal{L}(\boldsymbol{\theta}_t)$. In our experiments we use $\sum_t \omega_t = 1$.

By appropriately choosing the weights $\{\omega_t\}$, we can interpolate between our two notions of tunability. In the extreme case where we are only interested in the peak performance of the optimizer, we can set $\omega_T = 1$ and set the other weights to zero. In the opposite extreme case where we are interested in the "one-shot tunability" of the optimizer, we can set $\omega_1 = 1$.

In general, we can answer the question of "How well does the optimizer perform with a budget of $K$ runs?" by setting \impulseatk.

While the above weighting scheme is intuitive, merely computing the performance after expending HPO budget of $K$ does not consider the performance obtained after the previous $K-1$ iterations i.e. we would like to differentiate the cases where a requisite performance is attained by tuning an optimizer for $K$ iterations and another for $K_1$ iterations, where $K_1\gg K$.
Therefore, we employ three additional weighting schemes.
By setting $\omega_i \propto (T - i)$, our first one puts more emphasis on the earlier stages of the hyperparameter tuning process. We term this weighting scheme \emph{Cumulative Performance-Early} (\weightingearly). In contrast, the second weighting scheme, \emph{Cumulative Performance-Late} (\weightinglate) puts more emphasis on late stages of tuning, and thus on obtaining a better performance at a higher tuning cost: $\omega_i \propto i$. As a intermediate of the two, we also report a uniform weighting \emph{Cumulative Performance-Uniform} (\weightingunif) \space: $\omega_i = 1 / T$.

==> tunability_table_new.tex <==
\newcommand{\horizfigtemp}[2][]{%
  \begin{subtable}{0.4\linewidth}
    \resizebox{\textwidth}{!}{#2}\subcaption{#1}\end{subtable}}
\newcolumntype{Z}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{\hspace*{-\tabcolsep}}}
\newcommand{\tb}[1]{\textbf{#1}}

\begin{table}[t]
  \caption{Performance of various experiments. $\uparrow$ means higher values are better. $\downarrow$ means lower values are better}
  \label{tab:tunab_table}
  \horizfigtemp[FMNIST 2C2D. $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & \tb{91.3} & 91.4      & 91.6      & 99.0      \\
      \Adam      & \tb{91.3} & 91.5      & 91.8      & 98.0      \\
      \AdamLR    & \tb{91.3} & \tb{91.6} & \tb{91.9} & 96.0      \\
      \SGD       & 90.4      & 90.8      & 91.2      & 95.0      \\
      \SGDM     & 90.5      & 90.9      & 91.3      & \tb{97.0} \\
      \SGDMC     & 90.7      & 90.9      & 91.1      & 83.0      \\
      \SGDMCWC   & 90.7      & 90.9      & 91.1      & 45.0      \\
      \SGDMW     & 90.4      & 90.8      & 91.3      & \tb{97.0} \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[CIFAR 10. $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 76.4      & 77.1      & 77.9      & 95.0      \\
      \Adam      & 77.2      & 78.4      & 79.5      & 91.0      \\
      \AdamLR    & 78.8      & 79.4      & 80.0      & 94.0      \\
      \SGD       & 77.0      & 77.8      & 78.6      & 93.0      \\
      \SGDM      & 77.8      & 78.6      & 79.5      & 91.0      \\
      \SGDMC     & 78.6      & 79.4      & 80.1      & 94.0      \\
      \SGDMCWC   & \tb{81.1} & \tb{81.6} & \tb{82.0} & 95.0      \\
      \SGDMW     & 79.7      & 80.4      & 81.2      & 94.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[CIFAR 100. $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 30.4      & 31.8      & 33.1      & 63.0      \\
      \Adam      & 39.4      & 42.2      & 45.1      & 40.0      \\
      \AdamLR    & \tb{42.2} & 43.0      & 43.8      & 71.0      \\
      \SGD       & 31.8      & 34.2      & 36.6      & 35.0      \\
      \SGDM      & 40.6      & \tb{43.3} & \tb{46.0} & 50.0      \\
      \SGDMC     & 42.1      & \tb{43.3} & 44.5      & 82.0      \\
      \SGDMCWC   & 39.2      & 40.3      & 41.5      & 78.0      \\
      \SGDMW     & 33.5      & 37.2      & 41.0      & 23.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[IMDB. $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 84.3      & 84.8      & 85.3      & 97.0      \\
      \Adam      & 83.6      & 84.5      & 85.5      & 93.0      \\
      \AdamLR    & \tb{85.8} & \tb{86.0} & \tb{86.3} & 70.0      \\
      \SGD       & 68.1      & 69.3      & 70.5      & 81.0      \\
      \SGDM      & 74.3      & 75.9      & 77.5      & 72.0      \\
      \SGDMC     & 79.3      & 80.1      & 81.0      & 88.0      \\
      \SGDMCWC   & 78.8      & 79.4      & 80.0      & 68.0      \\
      \SGDMW     & 75.7      & 77.1      & 78.6      & 86.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[WRN-16(4). $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 94.8      & 94.9      & 95.0      & 10.0      \\
      \Adam      & 94.5      & 94.8      & 95.2      & 71.0      \\
      \AdamLR    & 95.1      & 95.3      & 95.4      & 98.0      \\
      \SGD       & 94.6      & 94.9      & 95.2      & 98.0      \\
      \SGDM      & 94.8      & 95.2      & \tb{95.6} & 98.0      \\
      \SGDMC     & 94.9      & 95.1      & 95.3      & 52.0      \\
      \SGDMCWC   & \tb{95.2} & \tb{95.4} & 95.5      & 98.0      \\
      \SGDMW     & 95.0      & 95.2      & 95.3      & 36.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[Char-RNN. $\uparrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 55.6      & 56.2      & 56.7      & 95.0      \\
      \Adam      & 54.4      & 55.7      & 57.0      & 87.0      \\
      \AdamLR    & \tb{56.9} & \tb{57.2} & 57.5      & 97.0      \\
      \SGD       & 40.3      & 42.5      & 44.6      & 47.0      \\
      \SGDM      & 51.4      & 54.0      & 56.5      & 59.0      \\
      \SGDMC     & 55.6      & 57.0      & \tb{58.3} & 87.0      \\
      \SGDMCWC   & 54.2      & 55.6      & 57.0      & 85.0      \\
      \SGDMW     & 45.1      & 48.2      & 51.2      & 32.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[FMNIST-VAE. $\downarrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 25.5      & 24.7      & 24.0      & 91.0      \\
      \Adam      & 26.0      & 24.8      & 23.7      & 90.0      \\
      \AdamLR    & \tb{24.6} & \tb{24.0} & \tb{23.5} & 95.0      \\
      \SGD       & 26.2      & 25.5      & 24.8      & 94.0      \\
      \SGDM      & 26.2      & 25.4      & 24.6      & 90.0      \\
      \SGDMC     & 28.6      & 26.7      & 24.9      & 75.0      \\
      \SGDMCWC   & 27.9      & 26.4      & 24.8      & 88.0      \\
      \SGDMW     & 26.5      & 25.7      & 24.8      & 91.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[MNIST-VAE. $\downarrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 30.3      & 29.4      & 28.4      & 92.0      \\
      \Adam      & 33.2      & 31.2      & 29.1      & 80.0      \\
      \AdamLR    & \tb{29.2} & \tb{28.6} & \tb{27.9} & 83.0      \\
      \SGD       & 53.3      & 53.1      & 52.9      & 98.0      \\
      \SGDM     & 36.0      & 32.9      & 29.9      & 58.0      \\
      \SGDMC     & 54.1      & 53.5      & 53.0      & 95.0      \\
      \SGDMCWC   & 54.0      & 53.5      & 53.0      & 94.0      \\
      \SGDMW     & 34.6      & 32.2      & 29.8      & 65.0      \\
      \bottomrule
    \end{tabular}
  }
  \horizfigtemp[Quadratic deep. $\downarrow$]{
    \begin{tabular}{lrrZZ}
      \toprule
      Optimizer & CPE       & CPU       & CPL       & Sharpness \\
      \midrule
      \Adagrad   & 91.5      & 89.6      & 87.6      & 66.0      \\
      \Adam      & 94.8      & 92.1      & 89.4      & 75.0      \\
      \AdamLR    & 91.2      & 89.5      & 87.7      & 93.0      \\
      \SGD       & 90.5      & 89.6      & 88.7      & 6.0       \\
      \SGDM      & 89.5      & 88.7      & 87.9      & 30.0      \\
      \SGDMC     & 89.6      & 88.6      & \tb{87.5}      & 95.0      \\
      \SGDMCWC   & \tb{88.6} & \tb{88.4} & 88.1 & 16.0      \\
      \SGDMW     & 89.3      & 88.9      & 88.4      & 14.0      \\
      \bottomrule
    \end{tabular}
  }
\end{table}


==> tunability_tables_epochs.tex <==

\begin{table*}[t]
  \caption{Performance of various experiments.}
  \label{tab:tunab_table}
  \horizfigtemp[FMNIST 2C2D. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  22.6 &  52.1 &  79.4 &  90.1 &  91.1 &  91.3 &  91.4 &  91.5 &  88.3 &  89.8 &  91.4 \\
      Adam &  48.8 &  67.5 &  80.6 &  90.3 &  91.4 &  91.7 &  91.8 &  91.8 &  89.5 &  90.6 &  91.7 \\
 AdamDecay &  60.0 &  75.4 &  88.0 &  91.5 &  91.7 &  91.8 &  91.8 &  91.8 &  90.5 &  91.1 &  91.8 \\
    AdamLR &  64.3 &  75.5 &  85.4 &  91.4 &  91.7 &  91.8 &  91.8 &  91.9 &  90.4 &  91.1 &  91.8 \\
       SGD &   8.0 &  63.0 &  67.8 &  87.9 &  89.8 &  90.6 &  91.0 &  91.1 &  86.7 &  88.8 &  90.8 \\
  SGDDecay &  43.8 &  71.3 &  84.0 &  90.6 &  91.2 &  91.3 &  91.4 &  91.4 &  89.3 &  90.3 &  91.4 \\
      SGDM &  26.4 &  60.7 &  65.5 &  87.7 &  89.8 &  90.8 &  91.1 &  91.2 &  87.0 &  89.0 &  90.9 \\
     SGDMC &  33.2 &  67.4 &  78.6 &  89.7 &  90.7 &  91.0 &  91.1 &  91.1 &  88.4 &  89.7 &  91.0 \\
   SGDMCWC &  29.6 &  69.0 &  81.0 &  90.1 &  90.8 &  91.0 &  91.1 &  91.1 &  88.6 &  89.8 &  91.0 \\
     SGDMW &  26.4 &  66.2 &  71.4 &  87.8 &  89.8 &  90.7 &  91.0 &  91.2 &  87.4 &  89.1 &  90.9 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[CIFAR 10. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  17.0 &  51.4 &  62.1 &  73.7 &  76.4 &  77.3 &  77.6 &  77.8 &  74.4 &  75.9 &  77.5 \\
      Adam &  29.0 &  50.6 &  61.4 &  74.6 &  77.5 &  78.8 &  79.4 &  79.6 &  75.9 &  77.5 &  79.2 \\
 AdamDecay &  32.4 &  57.4 &  74.5 &  78.3 &  79.6 &  80.3 &  80.6 &  80.8 &  78.3 &  79.4 &  80.5 \\
    AdamLR &  44.1 &  63.5 &  73.0 &  78.1 &  79.3 &  79.7 &  79.9 &  80.0 &  78.1 &  79.0 &  79.9 \\
       SGD &  23.7 &  43.5 &  50.2 &  69.8 &  75.2 &  77.2 &  78.0 &  78.3 &  73.2 &  75.5 &  77.7 \\
  SGDDecay &  19.1 &  50.2 &  68.8 &  78.7 &  81.5 &  82.5 &  83.1 &  83.4 &  79.4 &  81.2 &  83.0 \\
      SGDM &  31.7 &  47.7 &  54.8 &  71.2 &  76.6 &  78.2 &  78.9 &  79.2 &  74.7 &  76.7 &  78.7 \\
     SGDMC &  35.1 &  47.7 &  55.1 &  72.6 &  77.9 &  79.2 &  79.7 &  79.9 &  75.8 &  77.7 &  79.5 \\
   SGDMCWC &  20.1 &  45.8 &  60.0 &  76.4 &  80.4 &  81.5 &  81.8 &  81.9 &  77.9 &  79.7 &  81.6 \\
     SGDMW &  13.8 &  36.5 &  54.8 &  72.4 &  77.8 &  80.0 &  80.8 &  81.1 &  75.5 &  78.0 &  80.5 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[CIFAR 100. Higher the better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &    1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  4.6 &  16.0 &  22.2 &  26.8 &  29.5 &  31.3 &  32.6 &  33.2 &  29.6 &  31.0 &  32.4 \\
      Adam &  2.0 &  11.6 &  18.0 &  24.3 &  32.3 &  38.4 &  42.3 &  44.0 &  34.6 &  38.1 &  41.7 \\
 AdamDecay &  5.8 &  23.0 &  29.2 &  33.2 &  35.2 &  36.3 &  37.0 &  37.1 &  34.7 &  35.7 &  36.8 \\
    AdamLR &  9.3 &  28.9 &  36.4 &  40.1 &  41.6 &  43.3 &  43.8 &  43.9 &  41.4 &  42.5 &  43.6 \\
       SGD &  1.9 &   6.9 &  10.5 &  14.2 &  18.0 &  24.0 &  28.9 &  32.0 &  21.9 &  25.3 &  28.6 \\
  SGDDecay &  3.3 &  15.7 &  21.8 &  29.4 &  35.4 &  39.1 &  40.7 &  41.2 &  35.7 &  38.0 &  40.3 \\
      SGDM &  2.5 &  11.3 &  15.9 &  20.4 &  25.6 &  33.4 &  39.9 &  42.3 &  30.6 &  34.7 &  38.9 \\
     SGDMC &  2.7 &  18.1 &  23.1 &  29.1 &  34.3 &  40.6 &  43.0 &  43.8 &  36.7 &  39.6 &  42.4 \\
   SGDMCWC &  2.2 &  15.8 &  21.2 &  27.1 &  31.3 &  37.1 &  39.3 &  40.2 &  33.7 &  36.3 &  38.9 \\
     SGDMW &  1.5 &   7.1 &  10.0 &  12.6 &  17.1 &  23.5 &  29.6 &  33.7 &  21.6 &  25.4 &  29.2 \\
\bottomrule
\end{tabular}

  }
  \horizfigtemp[IMDB. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  51.7 &  66.0 &  72.1 &  82.4 &  84.2 &  84.9 &  85.2 &  85.3 &  82.8 &  83.9 &  85.1 \\
      Adam &  52.3 &  60.4 &  72.1 &  81.0 &  83.1 &  84.1 &  84.9 &  85.4 &  82.0 &  83.4 &  84.8 \\
 AdamDecay &  30.0 &  45.3 &  55.2 &  81.3 &  85.0 &  86.1 &  86.5 &  86.8 &  81.9 &  84.1 &  86.3 \\
    AdamLR &  63.9 &  73.0 &  77.2 &  85.1 &  85.9 &  86.1 &  86.3 &  86.3 &  84.8 &  85.5 &  86.2 \\
       SGD &  25.4 &  41.1 &  59.0 &  64.0 &  66.7 &  68.4 &  69.6 &  70.2 &  65.9 &  67.6 &  69.4 \\
  SGDDecay &  12.1 &  20.0 &  33.5 &  67.2 &  74.1 &  78.5 &  81.0 &  81.8 &  72.4 &  76.4 &  80.3 \\
      SGDM &  30.5 &  42.9 &  61.2 &  68.3 &  72.0 &  74.4 &  76.2 &  77.2 &  71.6 &  73.8 &  76.0 \\
     SGDMC &  43.9 &  55.0 &  69.1 &  75.6 &  78.6 &  80.3 &  80.9 &  81.0 &  77.8 &  79.2 &  80.7 \\
   SGDMCWC &   9.2 &  16.2 &  24.0 &  67.6 &  73.8 &  77.3 &  78.8 &  79.4 &  70.5 &  74.4 &  78.3 \\
     SGDMW &   6.2 &  12.4 &  18.0 &  58.6 &  64.5 &  70.3 &  74.8 &  76.9 &  63.9 &  69.0 &  74.1 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[WRN-16(4). Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  66.3 &  82.6 &  90.0 &  94.8 &  95.1 &  95.1 &  95.1 &  95.1 &  93.9 &  94.5 &  95.1 \\
      Adam &  33.9 &  65.8 &  83.3 &  94.1 &  95.0 &  95.1 &  95.1 &  95.2 &  92.5 &  93.8 &  95.1 \\
 AdamDecay &  35.3 &  81.0 &  94.6 &  95.2 &  95.3 &  95.3 &  95.3 &  95.3 &  93.8 &  94.5 &  95.3 \\
    AdamLR &  74.4 &  84.9 &  94.2 &  95.3 &  95.3 &  95.4 &  95.4 &  95.4 &  94.5 &  94.9 &  95.4 \\
       SGD &  42.2 &  66.4 &  80.1 &  90.3 &  94.8 &  95.0 &  95.1 &  95.2 &  92.1 &  93.6 &  95.0 \\
  SGDDecay &  26.3 &  75.1 &  87.9 &  94.8 &  95.3 &  95.4 &  95.4 &  95.4 &  93.0 &  94.2 &  95.3 \\
      SGDM &  48.9 &  67.3 &  79.7 &  92.2 &  95.0 &  95.3 &  95.4 &  95.5 &  92.5 &  93.9 &  95.3 \\
     SGDMC &  55.3 &  75.8 &  85.3 &  91.8 &  95.1 &  95.3 &  95.3 &  95.3 &  93.1 &  94.2 &  95.2 \\
   SGDMCWC &  24.4 &  73.4 &  83.5 &  90.6 &  95.3 &  95.4 &  95.5 &  95.5 &  92.5 &  93.9 &  95.4 \\
     SGDMW &  24.9 &  60.7 &  80.6 &  92.6 &  95.1 &  95.3 &  95.4 &  95.4 &  92.1 &  93.7 &  95.3 \\
\bottomrule
\end{tabular}

  }
  \horizfigtemp[Char-RNN. Higher is better]{

\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  10.4 &  41.6 &  50.4 &  54.6 &  55.8 &  56.2 &  56.6 &  56.7 &  54.5 &  55.5 &  56.5 \\
      Adam &   9.9 &  32.1 &  42.6 &  51.0 &  54.8 &  56.6 &  57.1 &  57.2 &  53.5 &  55.2 &  56.9 \\
 AdamDecay &   6.8 &  42.4 &  51.0 &  56.0 &  57.4 &  58.1 &  58.4 &  58.5 &  56.1 &  57.2 &  58.3 \\
    AdamLR &  12.3 &  46.0 &  53.7 &  56.4 &  57.1 &  57.3 &  57.4 &  57.5 &  55.8 &  56.6 &  57.4 \\
       SGD &   5.5 &  19.2 &  26.7 &  32.9 &  38.1 &  41.0 &  42.8 &  43.7 &  38.1 &  40.3 &  42.5 \\
  SGDDecay &   0.1 &  22.9 &  29.8 &  40.2 &  47.0 &  51.4 &  53.3 &  53.7 &  47.2 &  50.0 &  52.7 \\
      SGDM &   3.7 &  21.1 &  29.8 &  39.7 &  46.6 &  51.6 &  55.1 &  56.4 &  47.6 &  51.0 &  54.5 \\
     SGDMC &   1.5 &  25.2 &  35.3 &  47.7 &  54.2 &  57.3 &  58.1 &  58.4 &  52.9 &  55.3 &  57.8 \\
   SGDMCWC &   0.1 &  24.3 &  33.8 &  45.5 &  52.4 &  55.5 &  56.8 &  57.1 &  51.1 &  53.7 &  56.3 \\
     SGDMW &   3.8 &  19.0 &  25.5 &  33.3 &  40.2 &  45.5 &  48.7 &  50.5 &  41.7 &  44.9 &  48.2 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[FMNIST-VAE. Lower is better.]{

\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &      1 &      2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  129.6 &  108.5 &  73.9 &  47.5 &  31.2 &  24.8 &  24.3 &  24.2 &  35.4 &  30.2 &  25.0 \\
      Adam &   96.1 &   83.0 &  66.2 &  42.8 &  28.6 &  24.5 &  23.9 &  23.8 &  32.2 &  28.3 &  24.5 \\
 AdamDecay &  107.5 &   68.0 &  54.0 &  32.0 &  25.5 &  23.6 &  23.4 &  23.4 &  29.5 &  26.6 &  23.7 \\
    AdamLR &  107.9 &   77.1 &  60.1 &  34.2 &  25.6 &  23.6 &  23.5 &  23.5 &  29.9 &  26.9 &  23.8 \\
       SGD &  104.4 &   75.3 &  47.0 &  30.1 &  25.3 &  24.9 &  24.9 &  24.8 &  29.5 &  27.3 &  25.0 \\
  SGDDecay &   93.3 &   81.1 &  49.5 &  37.0 &  27.7 &  25.4 &  25.2 &  25.2 &  31.0 &  28.2 &  25.5 \\
      SGDM &  106.0 &   71.6 &  39.0 &  29.6 &  25.0 &  24.7 &  24.6 &  24.6 &  28.8 &  26.8 &  24.8 \\
     SGDMC &  100.0 &   80.3 &  55.6 &  38.5 &  28.0 &  24.9 &  24.8 &  24.7 &  31.2 &  28.2 &  25.1 \\
   SGDMCWC &  101.6 &   83.9 &  55.0 &  35.1 &  26.2 &  25.0 &  24.9 &  24.8 &  30.7 &  27.9 &  25.1 \\
     SGDMW &   89.4 &   69.4 &  42.5 &  28.8 &  25.0 &  24.9 &  24.8 &  24.8 &  28.5 &  26.7 &  24.9 \\
\bottomrule
\end{tabular}

  }
  \horizfigtemp[MNIST-VAE. Lower is better]{


\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &      1 &      2 &      4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  180.8 &  180.6 &  138.7 &  80.3 &  38.3 &  29.6 &  28.8 &  28.6 &  47.7 &  38.8 &  29.9 \\
      Adam &  131.8 &  112.3 &   93.5 &  53.9 &  38.8 &  32.8 &  29.7 &  29.1 &  42.1 &  36.4 &  30.7 \\
 AdamDecay &  167.2 &  158.4 &   72.2 &  42.7 &  29.1 &  27.7 &  27.5 &  27.5 &  38.4 &  33.2 &  28.0 \\
    AdamLR &  171.5 &  144.3 &  100.6 &  49.8 &  29.9 &  28.0 &  27.9 &  27.9 &  39.5 &  33.9 &  28.4 \\
       SGD &  125.7 &   75.9 &   64.0 &  53.4 &  52.9 &  52.9 &  52.9 &  52.9 &  55.7 &  54.3 &  53.0 \\
  SGDDecay &  110.0 &   76.8 &   65.4 &  55.0 &  53.0 &  52.9 &  52.9 &  52.9 &  55.6 &  54.3 &  53.0 \\
      SGDM &  117.7 &   86.9 &   63.5 &  49.1 &  42.8 &  36.6 &  31.4 &  29.6 &  41.7 &  37.0 &  32.3 \\
     SGDMC &   99.9 &   86.1 &   72.6 &  56.3 &  53.3 &  53.0 &  53.0 &  53.0 &  56.3 &  54.7 &  53.1 \\
   SGDMCWC &   94.2 &   80.5 &   66.1 &  55.1 &  53.1 &  53.0 &  52.9 &  52.9 &  55.4 &  54.2 &  53.0 \\
     SGDMW &  113.0 &   77.8 &   55.2 &  45.5 &  38.6 &  33.2 &  29.8 &  29.3 &  38.2 &  34.4 &  30.7 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[Quadratic deep. Lower is better]{

\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &      1 &      2 &      4 &      8 &    16 &    32 &    64 &   100 &    CPE &   CPU &   CPL \\
\midrule
   Adagrad &  211.1 &  205.3 &  169.2 &  105.6 &  92.1 &  88.6 &  87.9 &  87.6 &   99.8 &  94.1 &  88.4 \\
      Adam &  174.6 &  164.1 &  133.0 &  104.0 &  97.3 &  93.0 &  90.5 &  89.4 &   99.4 &  95.2 &  91.1 \\
 AdamDecay &  223.6 &  231.4 &  185.1 &  113.4 &  94.4 &  90.2 &  88.7 &  88.6 &  103.1 &  96.3 &  89.6 \\
    AdamLR &  212.6 &  206.0 &  155.7 &  103.9 &  91.0 &  88.1 &  87.7 &  87.7 &   98.5 &  93.4 &  88.2 \\
       SGD &  225.0 &  206.3 &  128.1 &   91.0 &  88.4 &  88.1 &  88.3 &  88.4 &   95.7 &  92.1 &  88.5 \\
  SGDDecay &  145.9 &  143.0 &   96.2 &   88.1 &  87.7 &  87.8 &  88.0 &  88.1 &   90.6 &  89.3 &  88.1 \\
      SGDM &  210.2 &  182.5 &  111.6 &   90.2 &  88.1 &  87.7 &  87.8 &  87.8 &   93.6 &  90.7 &  87.9 \\
     SGDMC &  181.2 &  154.4 &  104.2 &   89.0 &  87.8 &  87.7 &  87.7 &  87.7 &   91.9 &  89.9 &  87.8 \\
   SGDMCWC &  165.2 &  143.5 &   94.6 &   88.0 &  87.6 &  87.6 &  87.7 &  88.0 &   90.7 &  89.3 &  87.8 \\
     SGDMW &  190.7 &  160.1 &  101.0 &   89.0 &  88.0 &  87.8 &  87.9 &  88.1 &   92.2 &  90.1 &  88.1 \\
\bottomrule
\end{tabular}

  }
\end{table*}


==> tunability_tables_expected_test_performance.tex <==

\begin{table*}[t]
  \caption{Performance of various experiments.}
  \label{tab:tunab_table}
  \horizfigtemp[FMNIST 2C2D. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  86.6 &  89.7 &  90.9 &  91.2 &  91.4 &  91.5 &  91.6 &  91.6 &  91.3 &  91.4 &  91.5 \\
      Adam &  76.0 &  87.3 &  90.6 &  91.4 &  91.7 &  91.8 &  91.9 &  91.9 &  91.3 &  91.6 &  91.9 \\
 AdamDecay &  83.1 &  90.2 &  91.4 &  91.7 &  91.8 &  91.9 &  92.0 &  92.0 &  91.6 &  91.8 &  92.0 \\
    AdamLR &  79.3 &  89.2 &  91.4 &  91.7 &  91.9 &  92.0 &  92.0 &  92.1 &  91.6 &  91.8 &  92.0 \\
       SGD &  75.9 &  85.7 &  88.8 &  90.1 &  90.7 &  91.0 &  91.2 &  91.3 &  90.4 &  90.8 &  91.1 \\
  SGDDecay &  81.5 &  89.0 &  90.7 &  91.2 &  91.4 &  91.5 &  91.5 &  91.5 &  91.1 &  91.3 &  91.5 \\
      SGDM &  76.4 &  85.8 &  88.8 &  90.2 &  90.8 &  91.1 &  91.3 &  91.3 &  90.5 &  90.9 &  91.2 \\
     SGDMC &  76.5 &  87.2 &  90.2 &  90.8 &  91.0 &  91.1 &  91.2 &  91.2 &  90.7 &  90.9 &  91.2 \\
   SGDMCWC &  79.2 &  88.1 &  90.3 &  90.9 &  91.1 &  91.2 &  91.3 &  91.3 &  90.8 &  91.1 &  91.3 \\
     SGDMW &  78.7 &  86.3 &  88.9 &  90.2 &  90.8 &  91.1 &  91.3 &  91.4 &  90.5 &  90.9 &  91.2 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[CIFAR 10. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  54.9 &  66.9 &  73.4 &  76.1 &  77.2 &  77.7 &  78.0 &  78.1 &  76.6 &  77.2 &  77.9 \\
      Adam &  48.1 &  62.4 &  71.8 &  76.0 &  78.0 &  79.0 &  79.5 &  79.7 &  77.3 &  78.3 &  79.4 \\
 AdamDecay &  59.0 &  70.6 &  76.3 &  78.7 &  79.8 &  80.5 &  80.8 &  81.0 &  79.4 &  80.1 &  80.7 \\
    AdamLR &  57.8 &  70.7 &  76.6 &  78.6 &  79.4 &  79.8 &  80.0 &  80.0 &  78.8 &  79.4 &  79.9 \\
       SGD &  56.3 &  67.6 &  73.3 &  76.1 &  77.4 &  78.1 &  78.5 &  78.7 &  76.9 &  77.7 &  78.4 \\
  SGDDecay &  62.9 &  74.3 &  79.6 &  81.6 &  82.5 &  83.1 &  83.5 &  83.7 &  82.1 &  82.8 &  83.4 \\
      SGDM &  56.5 &  68.5 &  74.4 &  76.9 &  78.2 &  78.9 &  79.4 &  79.6 &  77.8 &  78.5 &  79.3 \\
     SGDMC &  57.3 &  70.0 &  76.2 &  78.3 &  79.2 &  79.8 &  80.2 &  80.3 &  78.8 &  79.4 &  80.1 \\
   SGDMCWC &  63.0 &  74.4 &  79.2 &  80.8 &  81.5 &  81.8 &  82.0 &  82.1 &  81.0 &  81.5 &  82.0 \\
     SGDMW &  56.3 &  68.2 &  75.3 &  78.8 &  80.3 &  81.0 &  81.3 &  81.4 &  79.6 &  80.4 &  81.2 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[CIFAR 100. Higher the better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  11.9 &  17.7 &  23.2 &  27.1 &  29.6 &  31.3 &  32.6 &  33.1 &  29.8 &  31.1 &  32.4 \\
      Adam &  10.3 &  16.1 &  23.3 &  30.8 &  37.2 &  41.3 &  43.9 &  45.2 &  38.1 &  40.8 &  43.5 \\
 AdamDecay &  16.9 &  24.2 &  30.1 &  33.5 &  35.3 &  36.4 &  37.1 &  37.3 &  35.1 &  36.0 &  36.9 \\
    AdamLR &  21.1 &  30.0 &  36.9 &  40.6 &  42.4 &  43.4 &  43.9 &  44.1 &  42.0 &  42.9 &  43.8 \\
       SGD &   9.8 &  13.9 &  18.7 &  24.0 &  29.3 &  33.3 &  35.8 &  36.9 &  30.6 &  33.0 &  35.3 \\
  SGDDecay &  17.1 &  24.8 &  32.3 &  37.3 &  39.7 &  40.9 &  41.6 &  42.0 &  39.2 &  40.4 &  41.5 \\
      SGDM &  12.9 &  19.1 &  26.3 &  33.5 &  39.1 &  42.7 &  45.0 &  46.1 &  39.8 &  42.2 &  44.6 \\
     SGDMC &  18.2 &  26.7 &  34.7 &  39.9 &  42.5 &  43.8 &  44.5 &  44.7 &  42.0 &  43.1 &  44.3 \\
   SGDMCWC &  17.6 &  25.2 &  32.1 &  36.7 &  39.1 &  40.4 &  41.2 &  41.6 &  38.8 &  39.9 &  41.1 \\
     SGDMW &   8.6 &  13.0 &  18.2 &  24.5 &  31.0 &  36.3 &  40.0 &  41.9 &  33.2 &  36.4 &  39.5 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[IMDB. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  71.4 &  78.1 &  82.2 &  83.9 &  84.7 &  85.1 &  85.3 &  85.4 &  84.4 &  84.8 &  85.3 \\
      Adam &  68.1 &  74.9 &  79.8 &  82.3 &  83.5 &  84.3 &  85.1 &  85.6 &  83.4 &  84.2 &  85.0 \\
 AdamDecay &  70.0 &  78.1 &  83.6 &  85.6 &  86.3 &  86.7 &  87.2 &  87.5 &  86.0 &  86.6 &  87.2 \\
    AdamLR &  77.9 &  82.4 &  84.5 &  85.6 &  86.1 &  86.3 &  86.5 &  86.5 &  85.9 &  86.2 &  86.4 \\
       SGD &  56.2 &  59.5 &  63.0 &  65.9 &  67.8 &  69.2 &  70.2 &  70.7 &  68.1 &  69.1 &  70.1 \\
  SGDDecay &  61.7 &  67.7 &  73.7 &  78.1 &  80.6 &  82.1 &  83.1 &  83.7 &  80.5 &  81.7 &  83.0 \\
      SGDM &  58.0 &  62.3 &  66.7 &  70.4 &  73.1 &  75.3 &  77.0 &  77.7 &  73.8 &  75.3 &  76.7 \\
     SGDMC &  61.8 &  67.5 &  72.8 &  76.9 &  79.4 &  80.6 &  81.0 &  81.1 &  79.0 &  79.9 &  80.8 \\
   SGDMCWC &  63.5 &  69.6 &  74.7 &  77.6 &  79.0 &  79.7 &  80.1 &  80.3 &  78.7 &  79.3 &  80.0 \\
     SGDMW &  56.1 &  59.9 &  64.9 &  70.6 &  75.2 &  77.6 &  78.6 &  78.9 &  75.2 &  76.7 &  78.3 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[WRN-16(4). Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  84.8 &  93.5 &  95.1 &  95.2 &  95.2 &  95.3 &  95.3 &  95.3 &  95.0 &  95.1 &  95.3 \\
      Adam &  70.5 &  87.0 &  93.9 &  95.0 &  95.1 &  95.2 &  95.3 &  95.3 &  94.5 &  94.9 &  95.3 \\
 AdamDecay &  79.6 &  91.7 &  94.9 &  95.3 &  95.4 &  95.5 &  95.6 &  95.6 &  95.1 &  95.3 &  95.6 \\
    AdamLR &  86.8 &  94.2 &  95.2 &  95.4 &  95.5 &  95.6 &  95.6 &  95.6 &  95.3 &  95.5 &  95.6 \\
       SGD &  79.1 &  91.4 &  94.4 &  94.9 &  95.1 &  95.2 &  95.3 &  95.3 &  94.7 &  95.0 &  95.3 \\
  SGDDecay &  84.3 &  93.3 &  95.1 &  95.4 &  95.5 &  95.5 &  95.5 &  95.6 &  95.2 &  95.4 &  95.5 \\
      SGDM &  78.8 &  91.4 &  94.6 &  95.1 &  95.3 &  95.4 &  95.5 &  95.6 &  94.9 &  95.2 &  95.5 \\
     SGDMC &  79.7 &  92.0 &  94.9 &  95.2 &  95.4 &  95.5 &  95.5 &  95.6 &  95.0 &  95.3 &  95.5 \\
   SGDMCWC &  84.1 &  93.5 &  95.2 &  95.4 &  95.5 &  95.6 &  95.7 &  95.7 &  95.3 &  95.5 &  95.7 \\
     SGDMW &  80.1 &  92.0 &  94.8 &  95.2 &  95.4 &  95.5 &  95.5 &  95.6 &  95.0 &  95.3 &  95.5 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[Char-RNN. Higher is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  38.9 &  48.2 &  53.4 &  55.3 &  56.0 &  56.4 &  56.6 &  56.7 &  55.6 &  56.1 &  56.6 \\
      Adam &  25.8 &  35.3 &  44.6 &  51.5 &  55.1 &  56.6 &  57.1 &  57.2 &  54.2 &  55.5 &  56.9 \\
 AdamDecay &  41.2 &  50.1 &  55.0 &  57.0 &  57.8 &  58.2 &  58.5 &  58.6 &  57.4 &  57.9 &  58.4 \\
    AdamLR &  45.1 &  52.6 &  55.8 &  56.9 &  57.2 &  57.4 &  57.5 &  57.5 &  56.9 &  57.2 &  57.4 \\
       SGD &  17.6 &  24.0 &  30.2 &  36.1 &  39.9 &  41.9 &  43.5 &  44.6 &  39.9 &  41.6 &  43.3 \\
  SGDDecay &  22.4 &  29.5 &  37.2 &  44.4 &  49.6 &  52.6 &  53.7 &  53.9 &  49.6 &  51.4 &  53.3 \\
      SGDM &  20.2 &  28.4 &  36.7 &  44.4 &  50.0 &  53.8 &  56.2 &  57.1 &  50.7 &  53.2 &  55.7 \\
     SGDMC &  26.0 &  35.8 &  45.5 &  53.0 &  56.7 &  58.0 &  58.3 &  58.4 &  55.5 &  56.8 &  58.2 \\
   SGDMCWC &  24.7 &  33.7 &  42.9 &  50.7 &  54.9 &  56.5 &  57.1 &  57.2 &  53.9 &  55.4 &  56.8 \\
     SGDMW &  17.8 &  24.1 &  30.7 &  37.7 &  43.6 &  47.4 &  49.9 &  51.4 &  44.4 &  47.0 &  49.6 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[FMNIST-VAE. Lower is better.]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  70.6 &  44.6 &  28.8 &  24.8 &  24.3 &  24.1 &  24.0 &  24.0 &  25.9 &  25.0 &  24.1 \\
      Adam &  66.7 &  43.8 &  30.2 &  25.4 &  24.2 &  23.9 &  23.7 &  23.6 &  25.7 &  24.7 &  23.7 \\
 AdamDecay &  53.9 &  32.4 &  24.5 &  23.6 &  23.5 &  23.4 &  23.4 &  23.4 &  24.3 &  23.8 &  23.4 \\
    AdamLR &  51.8 &  31.1 &  24.3 &  23.6 &  23.5 &  23.5 &  23.5 &  23.4 &  24.3 &  23.9 &  23.5 \\
       SGD &  62.7 &  40.5 &  28.6 &  25.3 &  25.0 &  24.9 &  24.8 &  24.8 &  26.2 &  25.6 &  24.9 \\
  SGDDecay &  86.8 &  64.7 &  46.2 &  34.0 &  27.2 &  25.4 &  25.2 &  25.2 &  29.8 &  27.6 &  25.4 \\
      SGDM &  66.8 &  43.4 &  29.6 &  25.3 &  24.7 &  24.7 &  24.6 &  24.6 &  26.3 &  25.4 &  24.6 \\
     SGDMC &  80.8 &  58.9 &  42.0 &  31.1 &  25.9 &  24.9 &  24.7 &  24.7 &  28.5 &  26.7 &  24.9 \\
   SGDMCWC &  77.1 &  55.0 &  38.7 &  29.0 &  25.4 &  24.9 &  24.8 &  24.7 &  27.9 &  26.4 &  24.9 \\
     SGDMW &  64.1 &  43.7 &  31.2 &  25.9 &  25.0 &  24.9 &  24.8 &  24.8 &  26.5 &  25.7 &  24.8 \\
\bottomrule
\end{tabular}

  }
  \horizfigtemp[MNIST-VAE. Lower is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &     1 &     2 &     4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  89.0 &  53.2 &  33.5 &  29.3 &  28.8 &  28.5 &  28.4 &  28.4 &  30.7 &  29.6 &  28.5 \\
      Adam &  86.9 &  58.7 &  43.9 &  36.6 &  31.7 &  29.5 &  29.0 &  28.8 &  33.1 &  31.1 &  29.2 \\
 AdamDecay &  64.9 &  37.7 &  28.9 &  27.8 &  27.6 &  27.5 &  27.4 &  27.4 &  28.6 &  28.0 &  27.4 \\
    AdamLR &  64.6 &  37.1 &  28.7 &  28.0 &  27.9 &  27.9 &  27.9 &  27.9 &  28.9 &  28.4 &  27.9 \\
       SGD &  70.9 &  56.5 &  53.2 &  52.9 &  52.9 &  52.9 &  52.9 &  52.9 &  53.4 &  53.2 &  52.9 \\
  SGDDecay &  84.0 &  68.3 &  58.1 &  53.6 &  52.9 &  52.9 &  52.9 &  52.9 &  54.3 &  53.6 &  52.9 \\
      SGDM &  71.0 &  55.3 &  49.1 &  45.1 &  39.9 &  34.0 &  30.0 &  29.1 &  37.1 &  34.0 &  30.9 \\
     SGDMC &  85.9 &  65.9 &  56.1 &  53.2 &  53.0 &  53.0 &  53.0 &  52.9 &  54.1 &  53.5 &  53.0 \\
   SGDMCWC &  83.3 &  64.9 &  55.9 &  53.2 &  53.0 &  53.0 &  52.9 &  52.9 &  54.0 &  53.5 &  53.0 \\
     SGDMW &  65.9 &  53.2 &  47.4 &  42.7 &  37.0 &  31.8 &  29.6 &  29.2 &  35.2 &  32.7 &  30.2 \\
\bottomrule
\end{tabular}
  }
  \horizfigtemp[Quadratic deep. Lower is better]{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 Optimizer &      1 &      2 &      4 &     8 &    16 &    32 &    64 &   100 &   CPE &   CPU &   CPL \\
\midrule
   Adagrad &  177.8 &  126.0 &   99.7 &  90.3 &  87.8 &  86.9 &  86.3 &  86.1 &  90.6 &  88.6 &  86.5 \\
      Adam &  167.3 &  120.8 &  104.9 &  99.5 &  95.2 &  91.7 &  89.6 &  88.8 &  95.4 &  92.7 &  90.0 \\
 AdamDecay &  199.3 &  138.3 &  104.8 &  93.2 &  89.4 &  87.9 &  87.3 &  87.1 &  92.8 &  90.2 &  87.5 \\
    AdamLR &  172.6 &  122.3 &   98.1 &  89.6 &  87.1 &  86.3 &  85.9 &  85.7 &  89.9 &  87.9 &  86.0 \\
       SGD &  168.8 &  110.1 &   90.9 &  87.8 &  87.1 &  86.8 &  86.6 &  86.5 &  89.3 &  88.0 &  86.7 \\
  SGDDecay &  132.4 &   96.4 &   88.5 &  87.1 &  86.5 &  86.2 &  86.0 &  85.9 &  87.5 &  86.8 &  86.0 \\
      SGDM &  148.2 &  103.5 &   90.3 &  87.6 &  86.7 &  86.2 &  85.9 &  85.8 &  88.2 &  87.1 &  86.0 \\
     SGDMC &  158.5 &  104.6 &   89.2 &  86.8 &  86.3 &  86.0 &  85.8 &  85.7 &  88.1 &  87.0 &  85.9 \\
   SGDMCWC &  137.3 &   96.8 &   88.2 &  86.7 &  86.2 &  86.0 &  85.8 &  85.8 &  87.4 &  86.7 &  85.9 \\
     SGDMW &  138.6 &   97.8 &   88.8 &  87.1 &  86.4 &  85.9 &  85.6 &  85.4 &  87.5 &  86.5 &  85.6 \\
\bottomrule
\end{tabular}
  }
\end{table*}

